Understanding and Improving Visual Prompting: A Label-Mapping Perspective

We revisit and advance visual prompting (VP), an input prompting technique for vision tasks. VP can reprogram a fixed, pre-trained source model to accomplish downstream tasks in the target domain by simply incorporating universal prompts (in terms of input perturbation patterns) into downstream data points. Yet, it remains elusive why VP stays effective even given a ruleless label mapping (LM) between the source classes and the target classes. Inspired by the above, we ask: How is LM interrelated with VP? And how to exploit such a relationship to improve its accuracy on target tasks? We peer into the influence of LM on VP and provide an affirmative answer that a better 'quality' of LM (assessed by mapping precision and explanation) can consistently improve the effectiveness of VP. This is in contrast to the prior art where the factor of LM was missing. To optimize LM, we propose a new VP framework, termed ILM-VP (iterative label mapping-based visual prompting), which automatically re-maps the source labels to the target labels and progressively improves the target task accuracy of VP. Further, when using a contrastive language-image pretrained (CLIP) model, we propose to integrate an LM process to assist the text prompt selection of CLIP and to improve the target task accuracy. Extensive experiments demonstrate that our proposal significantly outperforms state-of-the-art VP methods. As highlighted below, we show that when reprogramming an ImageNet-pretrained ResNet-18 to 13 target tasks, our method outperforms baselines by a substantial margin, e.g., 7.9% and 6.7% accuracy improvements in transfer learning to the target Flowers102 and CIFAR100 datasets. Besides, our proposal on CLIP-based VP provides 13.7% and 7.1% accuracy improvements on Flowers102 and DTD respectively. Our code is available at https://github.com/OPTML-Group/ILM-VP.

==> AChen/tex/approach.tex <==
\section{Methodology: Iterative Label Mapping}
%In this section, we will develop a new label mapping design approach, termed Iterative Label Mapping (\textbf{\ours}), which significantly improves AR performance. Different from one-shot frequency label mapping in \cite{tsai2020transfer}, we formalize AR as a Bi-level problem and optimize the input pattern and the label mapping function respectively in the inner loop and the outer loop.

% fail case
% analysis
% define f if
% clip (no data level, but prompt level) 30%, related

In this section, we first provide a warm up study on frequency LM (FLM). Based on the observation of post-training frequency mapping matrix, we then propose our method \ours, which progressively adjust LM function according to the learnt input pattern.
Later, we study the potential of LM function design on CLIP, a contrastive language–image pre-trained model. Despite CLIP's independence of source prediction labels, we still develop sample-wise LM (SLM) to help prompt selection to boost its performance.

\subsection{Warm up: Frequency LM}
Frequency LM was proposed in \cite{tsai2020transfer}, which targets on finding a label mapping function that is consistent with target task's source prediction response. This method feeds the target data (with zero padding) into the frozen classifier and collect the prediction frequency matrix. Based on this frequency matrix, we use a greedy approach to select the best naturally paired source labels and target labels, reflected as the most paired samples (samples belonging to class A in target data and are predicted as B in source network prediction). A similar method has been proposed in \cite{yen2021study}, which uses representative samples' prediction logits in each class instead of the whole dataset's prediction frequency.
Table\,\ref{tab: exp_main} shows us the significant improvements brought by FLM (compared with RLM and CLM), especially on datasets like OxfordPets (from $9.27\%$ to $62.85\%$).

Despite the huge success FLM has achieved, we doubt if FLM finds the best LM function. Intuitively we would like the chosen best paired source and target labels to stay the best paired after the training process of the input pattern. However, Figure\,\ref{fig: flm_post_mapping_matrix} shows that they are not best paired anymore. Furthermore, most of the target data are predicted to the same class by the source network (e.g. here most of CIFAR10 images are classified as \textit{pinwheel}, which is not a mapping source of any target class). With this interesting phenomenon, we raise a question:
\begin{center}
	\vspace*{-5.5mm}
	\setlength\fboxrule{0.1pt}
	\noindent\fcolorbox{black}[rgb]{0.85,0.9,0.95}{\begin{minipage}{0.98\columnwidth}
			%\begin{center}
				\vspace{-0.00cm}
                Can we ensure pre- and post-training LM to be the same?
				\vspace{-0.00cm}
		%	\end{center}
	\end{minipage}}
	\vspace*{-3.5mm}
\end{center}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{AChen/figs/flm_post_mapping_matrix.png}
    \caption{Post-training frequency matrix of FLM-VP, the rows refer to classes of CIFAR10 and the columns refer to classes of ImageNet. The left 10 columns are chosen mapping source (by pre-training FLM) of CIFAR10 classes respectively and the right 10 columns are the most predicted source classes.}
    \label{fig: flm_post_mapping_matrix}
\end{figure}

\subsection{Our Proposal: \textbf{\ours}}
Since a LM guided input pattern training is not enough to solve our problem, we believe that the input pattern and the LM function should be coupled at the training time.
To this end, we extend the LM design from a one-shot pre-training technique to an iterative dynamic process. We adopt the idea of FLM due to it's to-some-extent success of selecting naturally best paired classes. 



\subsection{On CLIP: Sample-wise LM}



==> AChen/tex/intro.tex <==
\section{Introduction}
\label{sec: intro}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{AChen/figs/ILM_first_figure_final.pdf}
    \caption{\Yuguang{Overview of our proposal: {\ours} introduces iterative label mapping (LM) based on the prior visual prompting (VP) methods, identifying more interpretable source-target mapping to help VP training and improve downstream task performance. \PYB{Can we add one sentence to mention improved accuracy (on average? Can refer to the table for details)} }}
    \label{fig: ILM_overview}
\end{figure}

Transfer learning is a well-known technique in machine learning (ML). When we humans learn new knowledge, we first try to compare and connect it with the knowledge we are already familiar with. The same idea is applied in transfer learning for ML: A neural network trained on a (usually large) dataset should be able to solve a \PY{relevant} downstream task with only slight modifications \PY{on the model weights}.
The most popular method used in transfer learning is finetuning, which takes the pre-trained source model as initialization and modifies either parts of the network or the whole network. The past few years have witnessed huge success in transfer learning, especially when the downstream dataset is limited in size.

Visual prompting (or adversarial reprogramming) \cite{bahng2022visual, elsayed2018adversarial, tsai2020transfer, yen2021study, chen2021adversarial, neekhara2018adversarial, neekhara2022cross} 
%lies in the transfer learning literature. 
\PY{is a new alternative to transfer learning.}
However, different from the 
\PY{standard finetuning approaches,}
%former methods, 
it leaves the pre-trained model intact. Instead of directly modifying the source network, VP integrates an input transformation (usually realized via input perturbations) and an output transformation (a function that maps source labels to target labels) to enable the frozen pre-trained network to accomplish the target task. Notably, this technique also enables black-box transfer learning (e.g., re-purposing  cloud API for ML) because it doesn't need the knowledge of architecture or the parameters of the pre-trained network \cite{tsai2020transfer}. %Therefore, on the good side, re-purposing a neural-network-based cloud API becomes possible and ML techniques can be applied to more practical settings. However, it's also true that these APIs may be maliciously reprogrammed and cause damage.

Despite the success prior works on VP have achieved (\textit{e.g.} new SOTA on medical datasets \cite{tsai2020transfer} and time series datasets \cite{yen2021study}), it remains elusive why VP can leverage knowledge hidden inside a frozen neural network. 
To understand this, we notice that there is a critical missing factor \PY{for improving VP} in relevant works: \PYB{This transition comes too fast; I think you should add some sentences like ``The current practice of VP is to use a fixed and pre-defined label mapping function between source and output labels, such as (make an example)''. Once readers understand how LM is implemented in existing works; we can then motivate its insufficiency}
\PY{How important is LM? Can we better design LM or co-train LM with VP design for improved performance?}
What can best guide the design of LM function and why. 
Although some \PY{prior arts}
%efficient techniques 
have been proposed to improve LM quality and thus the overall performance of the VP framwork\cite{tsai2020transfer, neekhara2022cross, yen2021study}, %no convincing explanation was ever given to justify the rationality of these methods.
\PY{their underlying mechanisms often lack proper explanations, and even worse, we will show that these LM strategies could be suboptimal to VP.}
%Therefore, we delve into the design of the LM function and the rationale behind. 

\PY{As shown in Fig. 1, to motivate the suboptimality in the current practice of LM,}
we adopt the idea in \cite{tsai2020transfer}, which uses a pre-prompt prediction frequency to determine the LM function. The pre-trained neural network finds the nearest classes for the target data with the initialization of the input pattern, and these classes are considered the easiest optimization targets. 
%However, we doubt the scope a pre-trained network can provide on the target dataset merely with a newly initialized input pattern. 
%Therefore, we compared the pre-prompt and post-prompt prediction frequency. 
\PY{However, we find significant inconsistency by investigating the patterns of pre-prompt and post-prompt prediction frequency of the same pre-trained network, which explains the degraded accuracy in VP due to the issue of suboptimal label mapping.}
%Not surprisingly, they are by no means similar. 
Based on this observation, we propose our novel method, which iteratively re-maps source labels to target labels based on the adjusted prediction frequency during the training process. The method overview is shown in Fig.\,\ref{fig: ILM_overview}. \PYB{Add that with our method, the mapping is more interpretable, and the VP accuracy also improves.} We summarize our \textbf{contributions} below:


\ding{172} (Formulation) We \PY{revisit} the algorithmic foundation of VP through the lens of bi-level optimization (\textbf{BLO}). The new formulation incorporates LM function from a pre-defined function as an optimization subroutine, providing the feasibility of co-optimizing the input pattern and the LM function.

\ding{173} (Algorithm) We propose a new {\ours} algorithm, which is built upon the aforementioned BLO formulation. Unlike computationally intensive standard BLO solvers, we simply use alternating optimization (\textbf{AO}) method. 

\ding{174} (Experiments) We conduct comprehensive experiments across 13 datasets and 3 architectures. We show that (i) {\ours} achieves significantly higher test accuracy than other existing VP methods on nearly all datasets, (ii) {\ours} possesses high interpretability merit which is missing in prior works, (iii) {\ours} can also be extended to CLIP model where there is no explicit LM process.


%We peer into a basic operation of VP --- label mapping (LM), to provide insights for this question. Further, based on our insights, we propose a novel LM method 




\iffalse
Transfer learning is a widely used methodology in machine learning (ML) which aims to tackle a new task by leveraging knowledge learnt from a source task. Current transfer learning methods mostly rely on finetuning a pretrained model on the target dataset \cite{pan2009survey}. Despite the tremendous success finetuning based transfer learning has achieved, it requires full access to the model trained on the source dataset. In practice, powerful fundamental models are not always as transparent as small models --- they usually hide behind commercial APIs provided by huge companies.
Can we leverage such source models for downstream tasks with themselves untouched? Inspired by adversarial attacks which maneuver model outputs by perturbing data inputs, \cite{elsayed2018adversarial} proposed \textit{Adversarial Reprogramming} (AR) which adds a learnable pattern to the input domain and a heuristic mapping to the output domain to fit a pretrained model into the target dataset.
Furthermore, \cite{tsai2020transfer} uses \textit{zeroth order optimization} to extend AR to blackbox settings, which was named as \textit{Blackbox Adversarial Reprogramming} (BAR). Through zeroth order gradient estimations, we could finally leverage a query-only fundamental model to solve downstream tasks.
Fig.\,\ref{fig:schematic_overview_of_AR_BAR} provides a schematic overview of AR and BAR.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{AChen/figs/bi_lm.pdf}
    \caption{Overview of Bi-LM}
    \label{fig:schematic_overview_of_AR_BAR}
\end{figure}

A large volume of existing works in the AR field focused on choices of application scenarios \cite{yang2021voice2series, chen2021adversarial, neekhara2022cross}. However, we doubt that whether or not the mapping in output domain counts, too.
In this paper, we revisit adversarial reprogramming to address two questions: (i) Is there any intrinsic connection between source label domain and target label domain? (ii) If the answer to (i) is affirmative, could we leverage these connections to design a better label mapping program?
\fi



==> AChen/tex/motivation.tex <==
\section{Problem Statement}
\label{sec: motivation}
In this section, we will begin by providing a brief background of AR, and then introduce the problem of our interest-\textit{label mapping} of adversarial reprogramming-which aims at revealing the connection between label spaces of source and target tasks and leveraging this connection to improve AR performance. Through a warm up study on existing label mapping methods, we empirically show that label mapping function is non-trivial to carefully design.

==> Sections_SLiu/Abstract_SLiu.tex <==
In this paper, we revisit and advance an emerging input prompting technique for vision tasks, called visual prompting (\textbf{VP}), which can \textbf{reprogram} a fixed, pre-trained source model to accomplish downstream tasks in the target domain by barely incorporating universal prompts (in terms of input perturbation patterns) into downstream datapoints. Yet, it remains elusive why VP stays effects even if the label mapping (\textbf{LM}) between the source prediction classes and the target data classes keeps random.  Inspired by the above, we ask: 
How is LM interrelated with VP? And how to explore and exploit such a relationship to explain the mechanism of VP and to improve its accuracy on target tasks?  %improve 
By peering into the influence of LM in VP, we provide an affirmative answer that a better `quality' of LM (assessed by mapping precision and explanation) can consistently improve the effectiveness of VP. This is in a sharp contrast to the existing work where the factor of LM was missing.
%neglected the importance of LM. % a missing factor 
Moreover,  we a new VP framework, termed {\textbf{\ours}} (\underline{i}terative \underline{l}abel \underline{m}apping-based \underline{v}isual \underline{p}rompting), which   automatically re-maps
the source task   labels to downstream task labels based on self-adjusted prediction frequencies and   thus    progressively improves the performance of VP. 
In addition, we conduct extensive experiments to exhibit the effectiveness of {\ours} in reprogramming source models, such as ImageNet-pretraining and CLIP (contrastive language–image pretraining),  to    \SL{[number]} target tasks. We show that {\ours} outperforms the state-of-the-art VP approach in a substantial margin, \textit{e.g.}, \SL{[xxx\%]}   and \SL{[xxx\%]}   accuracy improvement in transfer learning from ImageNet-pretraining   to the target datasets \SL{[xxx]} and \SL{[xxx]}. Furthermore, we show that the  proposed   LM approach can  be readily extended to improve the performance of {VP} using a  CLIP (contrastive language–image pretraining)-type source model by leveraging LM for   text prompt selection.


% In data-scarce machine learning domains (e.g. medical image classification), transfer learning has always been a powerful approach to address difficult tasks. However, it remains unclear how the knowledge from source data is transferred. Fortunately, a recent work \aochuan{Madry's data based perspective of transfer learning. Can we cite here?} provided us a view of influences of source task classes on downstream tasks: there exist positive and negative classes in source dataset which respectively improve and degrade downstream task performance. Inspired by this discovery, we delve into a scenario where source task classes are directly connected to downstream task classes: label mapping of visual prompting (or adversarial reprogramming). Through the lens of frequency mapping matrix, we develop a better label mapping method which iteratively re-maps source task labels to downstream task labels based on the prediction frequency. Compared with the existing one-shot frequency label mapping, our method gains significant accuracy improvement on multiple datasets. Furthermore, we leverage the analysis of explanation by example to reveal the connection between source and downstream task labels. In general, our work sheds light on (i) how to better leverage visual prompting for transfer learning by carefully designing the label mapping function; (ii) when and why transfer learning works given different source and downstream tasks.
